Momentum Approximation in Asynchronous Private Federated Learning

Asynchronous protocols have been shown to improve the scalability of federated learning (FL) with a massive number of clients. Meanwhile, momentum-based methods can achieve the best model quality in synchronous FL. However, naively applying momentum in asynchronous FL algorithms leads to slower convergence and degraded model performance. It is still unclear how to effective combinie these two techniques together to achieve a win-win. In this paper, we find that asynchrony introduces implicit bias to momentum updates. In order to address this problem, we propose momentum approximation that minimizes the bias by finding an optimal weighted average of all historical model updates. Momentum approximation is compatible with secure aggregation as well as differential privacy, and can be easily integrated in production FL systems with a minor communication and storage cost. We empirically demonstrate that on benchmark FL datasets, momentum approximation can achieve $1.15 \textrm{--}4\times$ speed up in convergence compared to naively combining asynchronous FL with momentum.

==> sections/introduction.tex <==
\section{Introduction}
Practical deployment of synchronous federated learning (FL)~\cite{mcmahan2017communication} encounters scalability and efficiency issues due to the requirement on global synchronization of clients' model updates, wherein the central aggregation are contingent upon the completion of local training and communication across all participating clients. 
Asynchronous FL (AsyncFL)~\cite{xie2019asynchronous,van2020asynchronous,park2021sageflow,chai2021fedat,nguyen2022federated,zhang2023no} improves the scalability by updating the model concurrently and independently at both the central server and the clients' side. 



On the other hand, momentum-based optimizers such as FedAvgM~\cite{hsu2019measuring} and FedAdam~\cite{reddi2020adaptive} greatly improve the model quality and convergence speed in synchronous FL. 
However, the stale clients' model updates in asynchronous aggregation hinders the convergence and utility of the model, particularly for the momentum-based optimizers.

\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{figs/baseline/flair_fedadam.png}
\caption{Negative impact of implicit momentum on FedAdam in AsyncFL on the FLAIR dataset. 
In SyncFL, FedAdam with momentum parameter $\beta>0.0$ converges slower than  FedAdam with $\beta=0.9$ while it is the opposite case in AsyncFL.}
\label{fig:implicit-momentum-results}
\end{figure}

%The nature of many asynchronous FL algorithms at the server are analogous to their counterparts in traditional asynchronous distributed training. For example, FedAvgM to asynchronous momentum SGD and FedAdam to asynchronous Adam.
The exacerbation in convergence of momentum-based optimizers have been studied in asynchronous SGD (AsyncSGD).
\citet{mitliagkas2016asynchrony} showed that AsyncSGD can be viewed as adding an implicit momentum term due to the stale gradients. 
For AsyncSGD with momentum, sophisticated tuning of the momentum parameter $\beta$ becomes critical \cite{zhang2017yellowfin}.
Compared to synchronous SGD, a smaller or even negative $\beta$ is preferred for AsyncSGD to counter implicit momentum. 
We observe the same phenomenon for momentum-based optimizers in AsyncFL. 
Figure~\ref{fig:implicit-momentum-results} shows that FedAdam with $\beta=0.5$ and $0.9$ underperforms $\beta=0$ case in AsyncFL while the pattern is the opposite in the synchronous setting.
%This issue resulting from stale gradient is further exacerbated for FedAdam and asynchronous Adam. 
%Numerous asynchronous FL algorithms and variants of FedAvg and FedAvgM \cite{xie2019asynchronous} \citesomething have been proposed to solve the straggler problem and reduce the influence of stale gradients to training performance. Particularly, \citet{nguyen2022federated} propose the FedBuff framework using buffered asynchronous aggregation to achieve scalability and compatibility with secure aggregation \citesomething and differential privacy \citesomething. To the best of our knowledge, FedBuff is the state-of-the-art AsyncFL algorithm in terms of both efficiency and performance at low privacy settings, and be competitive for high privacy settings. 
%To alleviate the influence of stale gradients to convergence, 
% FedBuff adopts a small buffer size ($C=10$) and 

Prior AsyncFL works down-scale the stale client updates before central aggregation 
to control the impact of staleness~\cite{xie2019asynchronous,park2021sageflow,nguyen2022federated}.
FedBuff also carefully tuned $\beta$ to be smaller for FedAvgM than the synchronous baseline.  
Nonetheless, they failed to fully address the implicit momentum issue in AsyncFL. 
It remains an open question \emph{how to effectively integrate asynchrony and momentum in FL to harness the advantages of scalability and improve model quality simultaneously?}

% \JW{We may explicitly mention that in the FedBuff paper, they still recommend to tune beta for different datasets and the best values also differ. This is an evidence that they didn't solve this problem. We can also mention that it is still an open question/problem: how to nicely/properly combine asynchrony and momentum? to get both benefits from scalability and better model quality.}
%More critically, a small buffer size makes it harder for adding strong privacy without destroying the model as larger noises would be required.

\textbf{Contributions. }  
In this paper, we focus on the FedBuff protocal~\cite{nguyen2022federated} which is the state of the art AsyncFL method and has been deployed in production systems~\cite{huba2022papaya,wang2023flint}. 
We demonstrate that implicit momentum introduces a bias in FedBuff and propose momentum approximation to address this issue. 
% The momentum update rule in synchronous settings can be viewed as a weighted average of historical updates using a momentum matrix $\mM$, which is uniquely determined by the value of momentum parameter $\beta$. 
% We approximate $\mM$ with a weighted average of the stale historical updates by estimating the ratio of the staleness in each iteration. 
% Our approximation allows for the momentum updating using stale gradients in a manner consistent with synchronous settings. 
Momentum approximation solves a least square problem in each FL iteration $t$ to find the optimal coefficients to weight the historical model updates before $t$, such that the weighted historical updates is close to the unbiased momentum updates.
We highlight the main contributions: 
\begin{itemize}[leftmargin=3mm]
\item Our method is compatible with any momentum-based federated optimizer and the convergence pattern behaves similar to synchronous FL. 
It resolves the need of extensively tuning of $\beta$ unlike prior works.
% We also provide a differentially private version of our method.
%Even better, our method allows using a large buffer size without affecting the convergence (due to increased staleness), e.g., $200$, which makes adding privacy easier. 
\item Our method is easy to implement in current FL production systems, and inherits all the benefits from FedBuff, such as its scalability, robustness and compatibility to privacy. 
%\JW{Here is a bit confusing. If we view FedBuff as an algorithm, then we must change something to make it better. May need some rephrasing.}
Our method incurs only a minor communication of a iteration number in addition to model updates, and storage cost of historical updates on the server side. 
%\JW{Maybe we don't need to mention this here? as it sounds like a drawback. We can also combine it with the second point.}
%, in contrast to significantly more communications of model weights or momentum in \citesomething.
% \item Our method allows using a large buffer size without affecting the convergence (due to increased staleness), e.g., $200$, which makes adding privacy easier. 
% To the best of our knowledge, we are the first to provide an asynchronous FedAdam algorithm. 
\item We empirically demonstrate that on two large-scale FL benchmarks, StackOverflow and FLAIR, our method achieves $1.15 \textrm{--}4\times$ speed up in convergence and $3\textrm{--}20\%$ improvements in utility. 
\end{itemize}


==> sections/methodology.tex <==

\section{Momentum Approximation in FedBuff}
\begin{algorithm}[t]
\caption{FedBuff with Momentum Approximation}
\label{alg:fedbuf}
\footnotesize

\begin{algorithmic}
\STATE \textbf{Inputs:} client Poisson sampling rate $q$, cohort size $C$, server optimizer \textsc{ServerOpt}, server learning rate $\eta$, number of FL iterations $T$, client local learning rate $\eta_l$, number, number of client local SGD steps $Q$
\WHILE{$t < T$}
\STATE $\gK_t\gets$ sampled clients with Poisson sampling rate $q$
\STATE Run \textsc{Client}($\param_t, t$) for $k\in\gK_t$ asynchronously
\IF{receives $\Delta_k(\param_{t-\tau(k)})$ and $\ve_{t-\tau(k)}$ from  $k$}
\STATE $\vx_t \gets \vx_t + \frac{1}{C}\Delta_k(\param_{t-\tau(k)})$
\STATE $\mW_t \gets \mW_t + \frac{1}{C}\ve_{t-\tau(k)}$
\ENDIF
\IF{received $C$ results in the buffer}
\IF{light-weight momentum approximation}
\STATE $u_t, v_t\gets$ solve \eqref{eq:obj_light-weight}
\STATE $\vm_t\gets v_t\vm_{t-1} + u_t\vx_t$
\ELSE
\STATE Save $\vx_t$ and load previous aggregates $\mX_{:t}$
\STATE $\mA_t\gets$ solve \eqref{eq:obj_online}
\STATE  $\vm_t\gets\mA_t\mX_{:t}$
\ENDIF
\STATE $\mH_{t}\gets$ update based on \textsc{ServerOpt}
\STATE $\param_{t+1}\gets\param_t - \eta \mH_t^{-1}\vm_t$
\STATE $\vx_{t+1}, \mW_{t+1} \gets \vzero$
\STATE $t\gets t + 1$
\ENDIF
\ENDWHILE
\STATE
\STATE \textbf{function} \textsc{Client}($\param, t$)
\begin{ALC@g}
\STATE $\param^\prime\gets$ run $Q$ SGD steps with $\eta_l$ on local data
\STATE $\ve_t\gets$ one-hot encoding of $t$
\STATE Upload $\Delta=\param - \param^\prime$ and $\ve_t$ to server
\end{ALC@g}
\end{algorithmic}
\end{algorithm}


In this section, we first introduce the implicit momentum issue~\cite{mitliagkas2016asynchrony} in FedBuff and demonstrate how it negatively impacts training, and then propose momentum approximation to alleviate this issue. 
We notice that the model updates in FedBuff can be expressed as a weighted average of staled gradients from all previous iterations, and the weight coefficients can be gathered from devices. 
The weighted average of historical gradients is similar to the exponential decay average used in momentum-based optimizers.
We propose to approximate the desired momentum update using the staleness weight coefficients to address the implicit momentum issue. 
An overview of our approach is outlined in Algorithm~\ref{alg:fedbuf}




\paragraph{Notation.}
For a matrix $\mA$, $\mA_{i}$ denotes the $i$th row of the matrix and $\mA_{:i, :i}$ denotes the sub-matrix with the first $i$ rows and columns of $\mA$.
We denote $\mX = [\vx_1, \vx_2, \dots, \vx_T]\in\R^{T\times d}$ as the sequence of model updates received by the server, and $\nabla\vf = [\nabla f(\param_1), \nabla f(\param_2), \dots, \nabla f(\param_T)]\in\R^{T\times d}$ as the true gradients of global objective at all iterations. 
We denote the FedBuff staleness as $\tau(k)$ for client $k$, i.e. $k$ is sampled at iteration $t-\tau(k)$ and their updates arrived at iteration $t$.
We let $\ve_i\in\{0, 1\}^T$  denote the binary one-hot encoding vector where all entries are 0 except for the $i$th entry being 1.

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figs/momentum_matrix.png}
\caption{Visualization of the desired momentum matrix $\mM$ ($\beta=0.9$), the implicit momentum matrix $\mM\mW$, the approximated momentum matrix $\mA\mW$, the staleness coefficient matrix $\mW$, and the solved weighting matrix $\mA$ in momentum approximation.}
\label{fig:implicit-momentum}
\end{figure*}



\subsection{Implicit Momentum Bias in Asynchronous FL}
In iteration $t$ of FedBuff, the aggregated model update $\vx_t$ is a weighted sum of model update from all previous iterations update to $t$:
\begin{align}
\E[\vx_t] &= \E[\frac{1}{C}\sum_{k\in\receivedclients_t} \Delta_k(\param_{t-\tau(k)})]  \nonumber
\\ &= \E[\sum_{i=1}^t  \frac{C_{t,i}}{C}\frac{1}{C_{t,i}} \sum_{k\in\gC_{t,i}} \Delta_k(\param_i)],
\end{align}
where $\gC_t$ is the set of $C$ clients arrived at iteration $t$, $\gC_{t,i}\subseteq\gC_t$ is the set of clients received $\param_i$ with staleness $\tau(k)=t-i$, $C_{t,i} = |\gC_{t,i}|$, and $\sum_{i=1}^t C_{t,i} = C$.

To simplify the notation, we focus on the case where each sampled client $k$ does 1 step of full gradient descent locally and thus $\E[\Delta_k(\param)] = \nabla F_k(\param)$. 
The general case where clients perform multiple steps of local SGD can be derived in a similar fashion.
We further assume that $\gC_{t,i}$ is a random subset of $\gK_i$ (the sampled clients at iteration $i\leq t$), and discuss the justification for the assumption as well as the case when $\gC_{t,i}$ is not a random subset in Appendix~\ref{app:biased}. 
With Proposition \ref{prop:unbiased} and a sufficiently large $m$:
\begin{align}
\E[\vx_t]  &= \sum_{i=1}^t  \frac{C_{t,i}}{C} \E_k[\frac{1}{C_{t,i}} \sum_{k\in\gC_{t,i}}  \nabla F_k(\param_i)] \nonumber
\\ &=\sum_{i=1}^t \frac{C_{t,i}}{C} \nabla f(\param_i).
\label{eq:xt}
\end{align}
We can rewrite the above as a linear operator on $\nabla\vf$:
\begin{align}
\E[\mX] &= \mW \nabla\vf, \,
\mW_{ij} = \begin{cases}
C_{i,j} / C & \text{if } i >= j\\
0 & \text{otherwise,}
\end{cases}
\end{align}
where $\mW\in\R^{T\times T}$ is a lower-triangular matrix denoting the fraction of stale model updates from previous iterations.
For synchronous FL, $\mW=\mI$ and thus $\E[\mX] = \nabla \vf$.

For momentum-based optimizers described in Section~\ref{sec:momentum},
the sequence of momentum updates $[\vm_1, \vm_2, \dots, \vm_T]$ applied in $\textsc{ServerOpt}$ can also be written as a linear operator $\mM\mX$ where $\mM\in \R^{T\times T}$ is a lower-triangular momentum matrix~\cite{denisov2022improved}\footnote{For momentum SGD optimizer without dampening, the values in the diagonal of $\mM$ are 1 instead of $1-\beta$.}:
\begin{align}
\mM_{ij} = \begin{cases}
\beta^{i-j}(1-\beta) & \text{if } i >= j\\
0 & \text{otherwise.}
\end{cases}
\end{align}
In FedBuff, $\E[\mM\mX] = \mM\mW\nabla\vf$ which has a bias of $(\mM\mW-\mM)\nabla\vf$ due to the \emph{implicit momentum} matrix $\mW$.
As visualized in Figure~\ref{fig:implicit-momentum}, $\mM\mW$ has a different scale than $\mM$.
The sequence of updates produced with $\mM\mW$ can be undesired and negatively impact the convergence as demonstrated in Figure~\ref{fig:implicit-momentum-results}. 

\subsection{Mitigating implicit momentum}
Previous work~\cite{mitliagkas2016asynchrony,zhang2017yellowfin} proposed to tune down or even use a negative value for the momentum parameter $\beta$ to mitigate the implicit momentum by posing strong assumptions on $\mW$.
Though it can be effective to some extent, finding the optimal $\beta$ for an arbitrary $\mW$ requires sophisticated hyper-parameter tuning, which is highly expensive in FL~\cite{khodak2021federated}.

We propose to directly correct the bias in FedBuff and approximate the desired $\mM\nabla\vf$ by weighting all the historical model updates, i.e., find a lower triangular matrix $\mA\in \R^{T\times T}$ such that $\E[\mA\mX] = \mA\mW\nabla\vf\approx \mM\nabla\vf$.
A natural objective would be to minimize $\lVert\mA\mW\nabla\vf - \mM\nabla\vf\rVert_F^2$ which is upper bounded by: $\lVert(\mA\mW- \mM)\nabla\vf\rVert_F^2 \leq  \lVert\mA\mW- \mM\rVert_F^2 \lVert\nabla\vf\rVert_F^2$. 
We thus consider to optimize the following objective to find the optimal $\mA$:
\begin{align}
    \min_{\mA\in \R^{T\times T}} &\lVert\mA\mW - \mM\rVert_F^2 
    \label{eq:obj}\\
    \text{subject to } & \mA_{ij} = 0, \forall j > i \nonumber.
\end{align}
Since $\mA$ is enforced to be a lower-triangular matrix, \eqref{eq:obj} can be solved online in each FL iteration $t$ with the following:
\begin{align}
\min_{\mA_t \in \R^{t}} &\lVert\mA_t\mW_{:t,:t} - \mM_{t,:t}\rVert_2^2. 
\label{eq:obj_online}
\end{align}
Solving \eqref{eq:obj_online} requires knowing $\mW$, which can be obtained by having each sampled client $k$ to upload a one-hot encoding $\ve_{t-\tau(k)} \in \{0,1\}^T$ of their model version $t-\tau(k)$\footnote{One-hot encoding of the model version is preferable to a single scalar value as it is compatible with secure aggregation and DP.}.
The server aggregates the one-hot encodings and updates $\mW$ online as:
$\mW_t = \frac{1}{C}\sum_{k\in\gC_t} \ve_{t-\tau(k)}$.
Sending the extra $\ve_{t-\tau(k)}$ adds a negligible communication cost as $T\ll d$ for common FL tasks.

\paragraph{Approximated momentum update.}
In each iteration $t$, the server receives $\vx_t, \mW_t$ from devices and saves them in local storage. 
The server then solves \eqref{eq:obj_online} using a common least square solver and  approximates the momentum updates as $\vm_t=\mA_t\mX_{:t}$, i.e., a linear combination of all historically received aggregates.
$\vm_t$ is then used to update the model as in \eqref{eq:update}.
 
\paragraph{Light-weight momentum approximation.}
The full approximation above requires a central server side storage cost of $\gO(Td)$ as $\vx_t$ from all iterations needs to be saved. 
This is usually not a concern for FL since $T$ is typically in the order of thousands and the model size $d$ is smaller to meet on-device resource constraints~\cite{xu2023federated,xu2023training}.

In the case of both $T$ and $d$ are high and the storage cost becomes a concern, we propose a light-weight approximation which has no extra storage cost than the original momentum update. 
Let $\va_t\in \R^t$ be an auxiliary vector defined recursively as:
\begin{align}
\va_1 = [u_1],~\va_t = [v_t\va_{t-1}, u_t].
\end{align}
Denote $\vm_t=\va_t\mX_{:t}$, then we can derive the following given that $\mW$ is a lower-triangular matrix:
\begin{align}
\E[\vm_t] 
&= [v_t\va_{t-1}, u_t]\mW_{:t,:t}\nabla\vf_{:t} \nonumber \\
&= v_t\va_{t-1}\mW_{:t-1,:t-1}\nabla\vf_{:t-1} + u_t\mW_{t,:t}\nabla\vf_{:t} \nonumber \\
&= \E[v_t\va_{t-1}\mX_{:t-1} + u_t\vx_t] \nonumber \\
&= v_t\E[\vm_{t-1}] + u_t\E[\vx_t].
\end{align}
In each iteration $t$, we solve the following:
\begin{align}
\min_{u_t, v_t\in\R} \lVert[v_t\va_{t-1}, u_t]\mW_{:t,:t} - \mM_{t,:t}\rVert_2^2,
\label{eq:obj_light-weight}
\end{align}
and approximate the momentum by maintaining one  buffer $\vm_t$ in the entire FL training where:
\begin{align}
\vm_t = v_t\vm_{t-1} + u_t\vx_t.
\label{eq:light-weight}
\end{align}
Note that \eqref{eq:light-weight} is similar to the original momentum update in \eqref{eq:momentum} except that $u_t, v_t$ are not constrained between $(0,1)$ and do not need to add up to 1.


\paragraph{Implicit momentum in preconditioner.}
For adaptive optimizers such as Adam~\cite{kingma2014adam} and RMSProp, the preconditioner $\mH_t$ is the square root of exponentially decaying average of the gradients' second moments:
\begin{align}
\mathrm{diag}(\mH_t)^2 \gets \beta^\prime\mathrm{diag}(\mH_t)^2 + (1-\beta^\prime) \vx_{t}^2.
\end{align}

The implicit momentum in $\vx_t$ could also impact the estimation of second moments. 
Nonetheless, preconditioner is known to be robust to delayed gradients~\cite{gupta2018shampoo,li2022differentially}. 
We leave the exploration of whether mitigating implicit momentum in the second moments is helpful to future work.

\subsection{Differentially private momentum approximation}
For a sampled client $k$ with staleness $\tau(k)$, the model updates $\Delta_k$ and model version one-hot encoding $\ve_{t-\tau(k)}$ are both sensitive information as they reveal the client's local data and their timing of participating FL.
We can use differential privacy (DP) mechanisms to protect both information. 

Let $\gamma$ be a scaling factor and $\vy_k = [\Delta_k, \gamma\ve_{t-\tau(k)}]$ be the payload that client $k$ intends to send to the server. 
We constrain the $\normltwo$ sensitivity of $\vy_k$ as:
\begin{align}
\bar{\vy}_k &= [\mathrm{clip}(\Delta_k, S_\Delta),  \gamma\ve_{t-\tau(k)}].
\end{align}
Then $\lVert\bar{\vy}_k\rVert_2\leq \sqrt{S_\Delta^2 + \gamma^2} = S$, and applying Gaussian Mechanism $\sum_k\bar{\vy}_k + \mathcal{N}(0, \sigma^2 S^2\mI_{d+T})$ satisfies $(\epsilon, \delta)$-DP as described in Section~\ref{sec:dp}.
By choosing  $\gamma=\frac{\sigma}{\sqrt{\xi^2 - \sigma^2}} S_\Delta$,
the Gaussian noise added to un-scaled $\sum_k \ve_{t-\tau(k)}$ is $\mathcal{N}(0, (\frac{\sigma}{\gamma} S)^2\mI_T))$ with standard deviation:
\begin{align}
\frac{\sigma}{\gamma}S &= \frac{\sigma}{\gamma} \sqrt{S_\Delta^2+\gamma^2} = \sqrt{\frac{\sigma^2(\xi^2-\sigma^2)}{\sigma^2} + \sigma^2} = \xi.
\label{eq:xi}
\end{align}
In practice, we tune $\xi > \sigma$ to balance the utility on $\sum_k \Delta_k$ and $\sum_k \ve_{t-\tau(k)}$. 
As momentum approximation is a post-processing~\cite{dwork2014algorithmic} on the private aggregates:
\begin{align}
\vx_t &= \frac{1}{C}[\sum_{k\in\gC_t}\mathrm{clip}(\Delta_k, S_\Delta) +\mathcal{N}(0, \sigma^2 S^2 \mI_d)], \\
\mW_t &= \frac{1}{C\gamma}[\sum_{k\in\gC_t}\gamma\ve_{t-\tau(k)}+\mathcal{N}(0, \sigma^2 S^2 \mI_T)],
\end{align} 
the approximated momentum $\vm_t$ also satisfies the same $(\epsilon, \delta)$-DP guarantee.
